Robustness of Excitations in the Random Dimer Model

The ground state solution of the random dimer model is at a critical point after, which has been shown with random link excitations. In this paper we test the robustness of the random dimer model to the random link excitation by imposing the maximum weight excitation. We numerically compute the scaling exponents of the curves arising in the model as well as the fractal dimension. Although strong finite size corrections are present, the results are compatible with that of the random link excitation. Furthermore, another form of excitation, the {\epsilon} - coupling excitation is studied. We find that near-optimal configurations belong to the same universality class as the travelling salesman problem. Thus, we confirm a conjecture on the scaling properties of combinatorial optimisation problems, for the specific case of minimum weight perfect matchings on 2-dimensional lattices. This document was submitted as my thesis project for the MSc Complex Systems Modelling course at King's College London in 2021. In particular, I would like to thank my supervisor, Dr Gabriele Sicuro for his insights and guidance.

==> Notes.tex <==

\section{To-do list}

\begin{itemize}
    \item Different boundary conditions -> change from periodic to anti periodic as in Bernard et al. 
    \item What other way is there to induce a rearrangement?
    \begin{itemize}
        \item Cut random link
        \item Cut specific link - max/min weight, edge that changes the max/min energy change
        \item change boundary condition from periodic to anti-periodic/closed
        \item "dilute" the graph - remove d\% of the links and then see how the overlap loop behaves.
        \item "dilute2" - remove d\% of the vertices.
        \item cut all links in one direction - same as boundary change
        \item cut vertex?
        \item cut two vertices?
    \end{itemize}
    \item Write out formulas for all variables e.g.Sw, Sqw, Th2w.
    
    \item Divergent correlations in spin glasses include in review
\end{itemize}

\section{Questions}
\begin{itemize}
    \item In Corberi 2018 et al, the bond diluted is model is studied, with the parameter d varied around. In a similar question to answer similar questions, can $\epsilon$ be varied and studied in the dimer model. 
\end{itemize}


\section{Literature Review}
\begin{itemize}
    \item Structure of the literature review.
    \begin{itemize}
        \item The random dimer model can be approached from 3 different perspectives
        \item From a mathematical point of view. This is equivalent to the infinite temperature setup, where all configurations have equal probabilities and the challenge is counting the number of them etc. Topics include: height functions, conformality, generalisations of the problem. Becomes very mathematical, don't understand most of it.
        \item From a physics point of view (zero temperature). Solutions center around maxima and it deals with describing the maxima. Topics include: correlations, criticality, conformality, scaling, perturbations etc.
        \item Computationally. Is it feasible to solve the problem, if so how quickly, algorithms, big O() notation, cavity method, blossom algorithm.
    \end{itemize}
    
    \item For more information look at this book (SLE, overview, 2D models) \url{https://arxiv.org/pdf/math-ph/0602049.pdf}
\end{itemize}

\section{Summary of papers}


\begin{itemize}

    \item 2003 Pagnani et al key points:
    \begin{itemize}
        \item Description of matching models.
        \item Explains and introduces $\epsilon$-coupling perturbation.
        \item Cavity method for Bethe lattice to investigate $\epsilon$ couplings overlap with ground state.
    \end{itemize}
    
    \item 2005 - Ardilla, Stanley - Tilings
    \begin{itemize}
        \item Overview in tilings therory
        \item Explanation and definitions, counting and existance.
    \end{itemize}
    
    \item  2001 A. K. Hartmann and A. P. Young Lower Critical Dimension of Ising Spin Glasses
    \begin{itemize}
        \item Ising spin-glass with different types of disorder - Gaussian and Bimodal (+-J)
        \item The authors clear up previous inconsistent results and show that for Gaussian model $T_c = 0$ and $ d_c > 2$, while for Bimodal (+-J) model they find marginal behaviour, which is expected at the lower critical dimension so they conclude that $d_c = 2$ in the second case. 
        \item The model:
        \begin{itemize}
            \item $H = - \sum_{\langle i,j \rangle} J_{ij}S_iS_j $
            \item two kinds of models.1. $J_{ij} Gaussian random variables$ with N(0,1) and 2. $J_{ij}= +-1$ with equal probability.
            \item $J_{ij}$ are quenched random variables and the sum runs over on the square lattice neighbours. 
            \item 2 different domains investigated: 1. switch the periodic domain wall to anti-periodic (it swaps the sign of the bonds) and 2. Add links the wrap around a free domain wall that induces a change in the ground state.
            \item Compare energies of perturbed system to original $\delta E = E_0^{pertb} - E_0$
            \item $\Delta E = (\delta E)_{av}$ which is the average over samples.
        \end{itemize}
        \item The change in the ground state is induced by a change of domain walls.
        \item At the lower critical dimension, one has $\theta = 0$ and expects an exponential divergence of the correlation length, where $\Delta E \approx L^{\theta}$.
        \item $\theta$ is negative (-0.282 and -0.266) for the different distributions which means that with increasing system size the change in energy decreases.
        \item They cannot rule out that domain-wall energy converges to small non-zero value, but find it unlikely.
        \item For the Gaussian model results are compatible with $T_c = 0$.
        \item +-J distribution is different. It does not seem to converge.
        \item Looking at the P($\Delta E = 0,2,4,6,8,10 $) they deduce that $\theta = 0$, and that $d_c = 0$.
        \item Most likely explanation is that correlation length diverges exponentially as $T \rightarrow 0$, like $e^{C/T}$
    \end{itemize}
    \item 2006 Amoruso et al. Conformal Invariance and SLE in Two-Dimensional Ising Spin Glasses
    \begin{itemize}
        \item The objective of this paper is to provide numerical evidence of translational and possibly conformal invariance in Ising Spin Glasses with Gaussian bond distribution. 
        \item Numerically study conformal invariance (CI) of domain walls.
        \item Present evidence that domain walls are Stochastic Loewner evolution processes in 2d.
        \item Conformal invariance test:
        \begin{itemize}
            \item CI requires that the probability of the number of times the domain wall crosses the dashed line in two different, but conformally invariant geometries to be equal.
            \item naive expectation would be that DW is less likely to cross the dashed line due to the reduced number of configurations after the slit.
            \item Conformal transformation between the two geometries: complicated function involveing modular elliptic function $\lambda(\tau)$
        \end{itemize}
        \item Conformal transformation from initial rectangle to new rectangle with two slits in the middle. 
        \item Defining the probabilities to cross the dashed line $p_1'$ and $p_2'$, they want to see that two are equal, which they do as system size increases.
        \item This implies that the DW is conformal.
        \item To investigate it further, they look at asymptotically, assuming a power law for the inverse system size dependence. And they find slow convergence.
        \item They suppose a fractal dimension for the domain wall $d_f$ for the number of crossing  $n>0$, and then find that both for even and odd number of crossing it fits the same curve. $d_f = 1.27$.
        \item This fractal dimension would indicate slow convergence for $n=0$.
        \item They confirm conformal invariance so next they investigate if the domain wals were also SLE processes. 
        \item DW is an SLE process if $\xi(t)$ is Brownian walk whose elements have an independent Gaussian distribution and variance $\kappa t$. Important as the central charge in conformal field theory. 
        \item The paper describes how to transform such a process to the upper half plane which is needed for SLE.
        \item they find that $\kappa = 2.1$, but also that the boundary conditions together with the finite system size does not properly satisfy SLE requirements. 
        \item If it is an SLE process than: $d_f = 1+ \frac{\kappa}{8}$, which is confirmed for the numerical estimates. 
        \item There exists an equation that links $d_f$ and $\theta$ numerical values. The authors than link the findings to conformal field theories. 
    \end{itemize}
    
    \item Bernard et al. Possible description of domain walls in two-dimensional spin glasses by stochastic Loewner evolutions
    \begin{itemize}
        \item They apply several tests to directly investigate if domain wall statistics converge to SLE.
        \item Compare the results to loop erased random walk ($SLE_2$) and minimum spanning tree (not SLE).
        \item The Hamiltonian used is $H = - \sum_{\langle i,j \rangle} J_{ij}S_iS_j $, with $J_{i j}$ Gaussian rvs with zero mean and $S_i \in \{-1,1\}$.
        \item Introduce perturbation to the system by changing the periodic boundary conditions to anti-periodic BCs, with the overlap being the domain wall.
        \item Triangular lattice with periodic (which is then changed to anti-) in the x direction and fixed (free) boundary conditions in the y direction. Cylinder shape for the grid - wraps around in 1 direction.
        \item They obtain numerical results that satisfies fractal dimension relationship: $L^{d_f}$. The results also confirm conformal invariance of DW in all cases.
        \item For a given SLE you can calculate the probabilty that the curve passes to the left of a point in the complex plane. Given scale invariance (true) this is used here to compare numerical estimates to the true value, which is subtracted from each other to show the difference from 0.
        \item subte differences for reflecting/absorbing boundary conditions for the LERW, even though $d_f$ remains the same.
        \item Another test that maps domain walls to dipolar SLEs passes the test, but it passes for minimum spanning tree as well, even though that's not SLE.
        \item domain Markov property is tested as well for the domain wall. Calculate the correlation between subsequenet values and they find that it decays rapidly by a factor of 100ish for n=2 to n=8.There has to be some correlation from the structure of the lattice, as it makes certain edges suboptimal in certain cases. 
        \item Domain Markov property requires a conditional probability condition for the curves which is numerically tested. They test it numerically but is inconclusive.
        \item read this for domain markov property and introduction on SLE
        \item \url{https://www.phys.ens.fr/~dbernard/Documents/Publications/Bernard_SLENotes_MSRI2012.pdf} 
    \end{itemize}
    
    \item 2018 Corberi et al. Fractal character of the phase ordering kinetics of a diluted ferromagnet
    \begin{itemize}
        \item They study the geometry of the bond diluted Ising model, in which pairwise interactions are randomly nullified with probability d - dilution. 
        \item The purpose of their study is to look at correlation timescales and to clarify inconsistent results in the literature and they study the bond diluted Ising model (BDIM) for richer results.
        \item Model:
        \begin{itemize}
            \item Hamiltonian is : $H = - \sum_{\langle i,j \rangle} J_{ij}S_iS_j $ with $P(J_{ij} = (1-d)\delta_{J_{ij}, J}+ d\delta_{J_{ij}, 0 }$
            \item Some equilibrium properties.
            \item Glauber transition rates are introduced to reverse spins.
            \item Periodic boundary conditions. 
            \item Observables they calculate:
            \begin{itemize}
                \item Average size of the growing domain or characteristic length R(t,d). It is the average size of the areas with uniform spins. 
                \item Wrapping probability is the probability that at time t a connected wrapping cluster of equally aligned spins is present in the system. Defined for all directions, like across x, y or around the torus. Prob of winding around the torus twice or more is negligible. 
                \item Pair connectedness function: the probability that two points at distance r belong to the same cluster -   $C(r,t,d)$.
            \end{itemize}
            \item The clean states - no disorder/dilution (d=0) is compared to models with different quenched disorder which is switched on.
            \item Simulations: 91x91 up to 512x512 system size, with $10^4 - 10^5 $ simulations. 
        \end{itemize}
        \item Average system size $R(t, d)$ increases with time until the system permits, which is when all spins are aligned.
        \item Wrapping probabilities are different for this model than for other ones, like the random field/random bond Ising model.
        \item Increasing dilution slows down the emergence of large clusters.
        \item Study the average squared winding angle of the spin cluster interfaces.
        \item Superuniversality property is not met at variance with refereneces.
        \item Conlcusion: They calculated the exponents for the observables at different dilutions and investigated them.
    \end{itemize}
    
    
    \item 2010 Wieland, Wilson Winding Angle Variance of Fortuin-Kasteleyn Contours
    \begin{itemize}
        \item 
    \end{itemize}
    
    \item 2001 Kenyon Conformal invariance of domino tilings
    \begin{itemize}
        \item Introduce height function that adds a third coordinate to the problem. 
        \item As we take the tilings of a region with smaller and smaller elements, there is a limit shape for the surface given by the height function. 
        \item Some areas are linear, meaning they are fixed.
        \item The behaviour of the surface is given by the inverse Kasteleyn matrix $K^{-1}$.
        \item The maths gets very difficult very quickly, like algebraic geometry.
        
        
        \item 2003 Kenyon An introduction to the dimer model
        \begin{itemize}
            \item Easier explanations of the dimer model than the one above. 
            \item Focuses on the artic circle graph.
        \end{itemize}
    \end{itemize}
    
    \item 2012 Kenyon Conformal invariance of loops in the double dimer model
    \begin{itemize}
        \item The loops in the double dimer model (overlap) are $SLE_4$ processes.
        \item Uses quaternions (generalisations of complex numbers: e.g: $a +b i +c j + d k$.
    \end{itemize}
    
    \item 2015 Caracciolo, Sicuro Scaling hypothesis for the Euclidean bipartite matching problem II. Correlation functions
    \begin{itemize}
        \item Bipartite matching problem on d dimensional hypertorus.
        \item 2 kinds of systems: Poisson-Poisson (all points are randomly draw) and grid-Poisson (1 set of points fixed to lattice points).
        \item Calculates average cost of optimal matching and correlation functions of optimal matching ray in the large N limit.
        \item The problem is expressed as an optimal transport problem: The Monge–Kantorovic problem. It involves the Laplace operator.
        \item The Laplace operator is expressed as Green's function.
        \item They derive analytical results for the correlation functions, without free parameters. 
        \item Numerical results then confirm their findinds in 1,2,3 dimensions.
        
        \item Summary of the article: \url{https://physics.aps.org/articles/v7/77}.
    \end{itemize}
    
    \item 2014 - Boniolo et al. - Correlation function for the Grid-Poisson Euclidean matching on a line and on a circle.pdf
    \begin{itemize}
        \item Looks at random assignment problem on grid-Poisson graph in d = 1 (easiest).
        \item One set of points fixed on semi integer points of line, others uniformly distributed.
        \item Very good overview of literature. 
        \item When the sizes of the 2 sets of points is approximately equal, nearest points might assymetric. E.g. nearest point to i is j, but for j its k. This creates frustration, which can induce correlations. 
        \item They focus on the study of correlations that emerge in the scaling region around the critical point.
        \item Model
        \begin{itemize}
            \item Introduce observables on each $\sigma_i$ on the points that is zero if not in the optimal matching (and other conditions) otherwise Ising spins, depending on the sign of the difference between the ith match. For example, if $b_i$ > $r_i$ then $\sigma_i = 1$.
            \item Critical exponent $p$ of the distance function is 1, and everything above 1 belongs to the same class so will look at 2.
            \item $t = p - 1$
        \end{itemize}
        \item Lot's of graphs but not really sure of the point of them. Why are they showing that exactly?
        \item Different scaling exponents for  $p<1$ and $p>1$ in the correlation function. 
        \item Analytical results starts off with introducing a random walk process. Where does it come from?
        \item Repeats the analysis for the periodic boundary condition too, where p=2 is exactly solvable. 
        \item Finds similar results as other literature numerical results match analytical ones.
        \item Fairly easy to understand with quite a lot of explanation in it. 
    \end{itemize}

    
\end{itemize}


Dear Daniel,
 
I attach a list of links to papers for the review.
Best
G
 
 
Criticality and conformality tests in spin glasses
https://arxiv.org/abs/cond-mat/0107308
https://arxiv.org/abs/cond-mat/0601711
https://arxiv.org/abs/1811.12675
+paper attached
 
 
Criticality and correlation functions in the assignment:
https://arxiv.org/abs/1403.1836
https://arxiv.org/abs/1504.00614
https://arxiv.org/abs/2012.13956
 
Conformality in the dimer covering (mathematically heavier, it is enough to summarize the results)
https://arxiv.org/abs/1105.4158
https://arxiv.org/abs/math-ph/9910002
 
Fractal curves in lattice models
https://arxiv.org/abs/1002.3220
 

==> self-assessment.tex <==
\newpage

{\large
Self-assessment:}

\begin{enumerate}
    \item Scientific quality:
    \begin{itemize}
        \item The project is to a high scientific quality, accurate numerical methods are used and we remained objective throughout the paper.
        \item Ideally the model should be simulated for larger system sizes with more instances, however that was infeasible due to computational limitations.
    \end{itemize}
    \item Breadth:
    \begin{itemize}
        \item The project is intended to be self-contained. For example lot of extra research into conformal invariance which was not covered on the course. 
        
        \item Since the project touches many fields, e.g. combinatorics, probability theory, statistical mechanics, algorithms three month was not enough to dive deep into all of them. 
    \end{itemize}
    \item Originality:
    \begin{itemize}
        \item Original work in chapter 4 that connects the problem at hand to a conjecture from 20 years ago. 
        
        \item Chapter 3 was largely based on a previous paper, however that was done on purpose. 
    \end{itemize}
    
    \item Presentation and logical structure of the report
    \begin{itemize}
        \item The report is well written, one topic follows from the previous one. Figures and tables are well designed with consistent colours throughout. 
        
        \item Ch. 2 is might be hard to understand for inexperienced readers, as the word limit forced dense text on complex mathematical topics. 
    \end{itemize}
\end{enumerate}

